Beyond Barker: Infant Mortality at Birth and Ischaemic Heart Disease in Older Age

Adverse conditions in early life can have consequential impacts on individuals' health in older age. In one of the first papers on this topic, Barker and Osmond 1986 show a strong positive relationship between infant mortality rates in the 1920s and ischaemic heart disease in the 1970s. We go 'beyond Barker', first by showing that this relationship is robust to the inclusion of local geographic area fixed effects, but not family fixed effects. Second, we explore whether the average effects conceal underlying heterogeneity: we examine if the infant mortality effect offsets or reinforces one's genetic predisposition for heart disease. We find considerable heterogeneity that is robust to within-area as well as within-family analyses. Our findings show that the effects of one's early life environments mainly affect individuals with the highest genetic risk for developing heart disease. Put differently, in areas with the lowest infant mortality rates, the effect of one's genetic predisposition effectively vanishes. These findings suggest that advantageous environments can cushion one's genetic risk of developing heart disease.

==> tab/BMI.tex <==
                    &\multicolumn{5}{c}{Body Mass Index}                                                                          \\\cmidrule(lr){2-6}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\midrule
IMR                 &      0.2193\sym{***}&                     &      0.1541\sym{***}&      0.1541\sym{***}&      0.0059         \\
                    &    (0.0336)         &                     &    (0.0243)         &    (0.0245)         &    (0.0119)         \\
\addlinespace
PGS BMI             &                     &      1.3291\sym{***}&      1.3277\sym{***}&      1.3274\sym{***}&      1.3148\sym{***}\\
                    &                     &    (0.0083)         &    (0.0084)         &    (0.0089)         &    (0.0090)         \\
\addlinespace
IMR $\times$ PGS BMI&                     &                     &                     &     -0.0552\sym{***}&     -0.0523\sym{***}\\
                    &                     &                     &                     &    (0.0118)         &    (0.0116)         \\
\midrule
Covariates          &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Principal components&          No         &         Yes         &         Yes         &         Yes         &         Yes         \\
District FEs        &          No         &          No         &          No         &          No         &         Yes         \\
Mean                &       27.42         &       27.42         &       27.42         &       27.42         &       27.42         \\
R$^2$               &        0.01         &        0.09         &        0.09         &        0.09         &        0.09         \\
No. of observations &      376911         &      376911         &      376911         &      376911         &      376911         \\


==> tab/CHD.tex <==
                    &\multicolumn{5}{c}{Coronary Heart Disease}                                                                   \\\cmidrule(lr){2-6}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
\midrule
IMR                 &      0.0087\sym{***}&                     &      0.0067\sym{***}&      0.0068\sym{***}&      0.0036\sym{***}\\
                    &    (0.0017)         &                     &    (0.0014)         &    (0.0014)         &    (0.0008)         \\
\addlinespace
PGS CHD             &                     &      0.0070\sym{***}&      0.0070\sym{***}&      0.0069\sym{***}&      0.0070\sym{***}\\
                    &                     &    (0.0005)         &    (0.0005)         &    (0.0004)         &    (0.0004)         \\
\addlinespace
IMR $\times$ PGS CHD&                     &                     &                     &      0.0031\sym{***}&      0.0031\sym{***}\\
                    &                     &                     &                     &    (0.0005)         &    (0.0005)         \\
\midrule
Covariates          &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Principal components&          No         &         Yes         &         Yes         &         Yes         &         Yes         \\
District FEs        &          No         &          No         &          No         &          No         &         Yes         \\
Mean                &        0.06         &        0.06         &        0.06         &        0.06         &        0.06         \\
R$^2$               &        0.04         &        0.04         &        0.04         &        0.04         &        0.04         \\
No. of observations &      357193         &      357193         &      357193         &      357193         &      357193         \\


==> tab/IHDcontrols.tex <==
                    &\multicolumn{2}{c}{Ischaemic Heart Disease}\\\cmidrule(lr){2-3}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
\midrule
IMR                 &      0.0007         &      0.0002         \\
                    &    (0.0049)         &    (0.0050)         \\
\addlinespace
PGS                 &      0.0218\sym{***}&      0.0218\sym{***}\\
                    &    (0.0033)         &    (0.0033)         \\
\addlinespace
IMR $\times$ PGS    &      0.0050\sym{*}  &      0.0050\sym{*}  \\
                    &    (0.0026)         &    (0.0026)         \\
\addlinespace
Illegitimacy Rate   &                     &     -0.0006         \\
                    &                     &    (0.0038)         \\
\addlinespace
Birth Rate          &                     &      0.0015         \\
                    &                     &    (0.0043)         \\
\addlinespace
Death Rate          &                     &      0.0021         \\
                    &                     &    (0.0035)         \\
\midrule
Additional covariates&          No         &         Yes         \\
R$^2$               &        0.57         &        0.57         \\
No. of observations &       33069         &       33069         \\


==> tab/IHDsquared.tex <==
                    &\multicolumn{2}{c}{Ischaemic Heart Disease}\\\cmidrule(lr){2-3}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
\midrule
IMR                 &      0.0007         &     -0.0005         \\
                    &    (0.0049)         &    (0.0048)         \\
\addlinespace
IMR squared         &                     &      0.0008         \\
                    &                     &    (0.0023)         \\
\addlinespace
PGS                 &      0.0218\sym{***}&      0.0220\sym{***}\\
                    &    (0.0033)         &    (0.0033)         \\
\addlinespace
PGS squared         &                     &      0.0058\sym{***}\\
                    &                     &    (0.0019)         \\
\addlinespace
IMR $\times$ PGS    &      0.0050\sym{*}  &      0.0051\sym{**} \\
                    &    (0.0026)         &    (0.0026)         \\
\midrule
R$^2$               &        0.57         &        0.57         \\
No. of observations &       33069         &       33069         \\


==> tab/IHDweighted.tex <==
                    &\multicolumn{2}{c}{Ischaemic Heart Disease}\\\cmidrule(lr){2-3}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
\midrule
IMR                 &      0.0007         &      0.0104         \\
                    &    (0.0049)         &    (0.0121)         \\
\addlinespace
PGS                 &      0.0218\sym{***}&      0.0303\sym{***}\\
                    &    (0.0033)         &    (0.0039)         \\
\addlinespace
IMR $\times$ PGS    &      0.0050\sym{*}  &      0.0071\sym{***}\\
                    &    (0.0026)         &    (0.0025)         \\
\midrule
R$^2$               &        0.57         &        0.63         \\
No. of observations &       33069         &       33063         \\


==> tab/cluster.tex <==
                    &\multicolumn{2}{c}{Ischaemic Heart Disease}\\\cmidrule(lr){2-3}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
\midrule
IMR                 &      0.0007         &      0.0007         \\
                    &    (0.0049)         &    (0.0046)         \\
\addlinespace
PGS                 &      0.0218\sym{***}&      0.0218\sym{***}\\
                    &    (0.0032)         &    (0.0032)         \\
\addlinespace
IMR $\times$ PGS    &      0.0050\sym{*}  &      0.0050         \\
                    &    (0.0030)         &    (0.0030)         \\
\midrule
R$^2$               &        0.57         &        0.57         \\
No. of observations &       33069         &       33069         \\


==> tab/descr.tex <==
                &     mean&       sd\\
\midrule
Ischaemic Heart Disease&    0.113&  (0.317)\\
Ischaemic Heart Disease&    0.444&  (0.497)\\
Body Mass Index &   27.418&  (4.761)\\
Years of education&   14.744&  (5.115)\\
\midrule
N               &   374720&         \\

